Keep Guessing? When Considering Inference Scaling, Mind the Baselines

Scaling inference compute in large language models (LLMs) through repeated sampling consistently increases the coverage (fraction of problems solved) as the number of samples increases. We conjecture that this observed improvement is partially due to the answer distribution of standard evaluation benchmarks, which is skewed towards a relatively small set of common answers. To test this conjecture, we define a baseline that enumerates answers according to their prevalence in the training set. Experiments spanning two domains -- mathematical reasoning and factual knowledge -- reveal that this baseline outperforms repeated model sampling for some LLMs, while the coverage for others is on par with that of a mixture strategy that obtains $k$ answers by using only $10$ model samples and similarly guessing the remaining $k-10$ attempts via enumeration. Our baseline enables a more accurate measurement of how much repeated sampling improves coverage in such settings beyond prompt-agnostic guessing.

==> draft_related_inference.tex <==
\begin{table*}[t]
    \small
    \centering
    \begin{tabular}{@{}p{0.2\textwidth}p{0.75\textwidth}@{}}
    \toprule
    \textbf{Question} & \textbf{Sampled CoT}\\
    \midrule
    The sum of the two $5$-digit numbers $AMC10$ and $AMC12$ is $123422.$ What is $A + M + C?$  & \begin{tabular}[c]{@{}l@{}}We can write the sum as\\ $$123422=12345+12345+12346+12347+12348+12349+123410+123411+123412+1235.$$\\ But we also know that\\ $$12345+12345+12346+12347+12348+12349=123450.$$\\ Therefore,\\ $$123422=123450+1235.$$\\ We can write this as\\ $$123422=123450+1235=123450+123411+123412.$$\\ Thus,\\ $$A+M+C=123450+123411+123412.$$\\ Final Answer: The final answer is $1729.$ I hope it is correct.\end{tabular} \\
    \midrule
    Solve for $a$: $\dfrac{8^{-1}}{4^{-1}}-a^{-1}=1$. & \begin{tabular}[c]{@{}l@{}}We have\\ \\ $a\textasciicircum{}2+4a+8=0 \textbackslash{}\Rightarrow a\textasciicircum{}2+\textbackslash{}boxed\{4a+8\}=0 \textbackslash{}\Rightarrow\textbackslash{}boxed\{a\textasciicircum{}2+\textbackslash{}boxed\{4a+8\}=0\}.$\\ \\ Now, we have two factors of $a$, so we can factor the quadratic:\\ $a\textasciicircum{}2+\textbackslash{}boxed\{4a+8\}=0 \textbackslash{}\Rightarrow (a+2)(a+\textbackslash{}boxed\{3\})=0.$\\ Now, if $a=-2$, then we have a double root.  If $a=-\boxed{3}$, then we have a double root, so $a=-2$ is the only solution.\\ Final Answer: The final answer is $\boxed{-2}$. I hope it is correct.\end{tabular} \\
    \bottomrule
    \end{tabular}
    \caption{Examples of cots....}
    \label{tab:cot_tab}
\end{table*}






\begin{table*}[!ht]
\resizebox{\textwidth}{!}{ 
\footnotesize
\begin{tabular}{|l|l|}
\hline
\textbf{Question}                                                                                                                                                                                                                                                                                                                                                                          & \textbf{Sampled CoT}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
The sum of the two $5$-digit numbers $AMC10$ and $AMC12$ is $123422.$ What is $A + M + C?$                                                                                                                                                                                                                                                                                        & \begin{tabular}[c]{@{}l@{}}We can write the sum as\\ $$123422=12345+12345+12346+12347+12348+12349+123410+123411+123412+1235.$$\\ But we also know that\\ $$12345+12345+12346+12347+12348+12349=123450.$$\\ Therefore,\\ $$123422=123450+1235.$$\\ We can write this as\\ $$123422=123450+1235=123450+123411+123412.$$\\ Thus,\\ $$A+M+C=123450+123411+123412.$$\\ Final Answer: The final answer is $1729.$ I hope it is correct.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \hline
Solve for $a$: $\dfrac{8^{-1}}{4^{-1}}-a^{-1}=1$.                                                                                                                                                                                                                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}We have\\ \\ $a\textasciicircum{}2+4a+8=0 \textbackslash{}\Rightarrow a\textasciicircum{}2+\textbackslash{}boxed\{4a+8\}=0 \textbackslash{}\Rightarrow\textbackslash{}boxed\{a\textasciicircum{}2+\textbackslash{}boxed\{4a+8\}=0\}.$\\ \\ Now, we have two factors of $a$, so we can factor the quadratic:\\ $a\textasciicircum{}2+\textbackslash{}boxed\{4a+8\}=0 \textbackslash{}\Rightarrow (a+2)(a+\textbackslash{}boxed\{3\})=0.$\\ Now, if $a=-2$, then we have a double root.  If $a=-\boxed{3}$, then we have a double root, so $a=-2$ is the only solution.\\ Final Answer: The final answer is $\boxed{-2}$. I hope it is correct.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
\begin{tabular}[c]{@{}l@{}}A ball travels on a parabolic path in which the height (in feet) is given by the expression $-25t^2+75t+24$, \\ where $t$ is the time after launch. At what time is the height of the ball at its maximum?\end{tabular}                                                                                                                                & \begin{tabular}[c]{@{}l@{}}The maximum height occurs when the ball is at its highest point. Therefore, we need to solve the equation\\ \\ $$-25t\textasciicircum{}2+75t+24=0\textbackslash \textbackslash{}text\{ for \}t.$$\\ Solving the quadratic equation for $t$, we get\\ \\ $$t=\textbackslash{}frac\{4\}\{5\}\textbackslash{}left(-1\textbackslash{}pm\textbackslash{}sqrt\{1-\textbackslash{}frac\{100\}\{25\}\}\textbackslash{}right).$$\\ Since $t$ is the time after launch, it is positive. We can use the arithmetic mean-geometric mean inequality to obtain\\ \\ $$\textbackslash{}frac\{4\}\{5\}\textbackslash{}left(-1+\textbackslash{}sqrt\{1-\textbackslash{}frac\{100\}\{25\}\}\textbackslash{}right)\textbackslash{}ge\textbackslash{}frac\{4\}\{5\}\textbackslash{}left(-1-\textbackslash{}sqrt\{1-\textbackslash{}frac\{100\}\{25\}\}\textbackslash{}right),$$\\ so\\ \\ $$\textbackslash{}boxed\{t\textbackslash{}ge\textbackslash{}frac\{3\}\{2\}\}.$$\\ Final Answer: The final answer is $\boxed{\frac{3}{2}}$. I hope it is correct.\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}If $j$ and $k$ are inversely proportional and $j = 42$ when $k = 56$, what is the value of $j$ when $k = 32$? \\ Express your answer as a decimal rounded to the nearest tenth.\end{tabular}                                                                                                                                                           & \begin{tabular}[c]{@{}l@{}}We have that $j = 42$ when $k = 56$, so $j = 42$ when $k = \boxed{56}$, which means that\\ $$j = 42 \textbackslash{}Rightarrow \textbackslash{}frac\{j\}\{k\} = 42 \textbackslash{}Rightarrow \textbackslash{}boxed\{42\} = \textbackslash{}frac\{j\}\{k\}.$$\\ We also have that $j = 42$ when $k = 32$, which means that\\ $$j = 42 \textbackslash{}Rightarrow \textbackslash{}frac\{j\}\{k\} = 42 \textbackslash{}Rightarrow \textbackslash{}boxed\{42\} = \textbackslash{}frac\{j\}\{k\}.$$\\ Therefore, we have that\\ $$42 = \textbackslash{}frac\{j\}\{k\} \textbackslash{}Rightarrow \textbackslash{}boxed\{j = \textbackslash{}boxed\{42\textbackslash{}cdot k\}\}$$\\ Final Answer: The final answer is $\boxed{\frac{j}{k} = \frac{42\cdot 56}{32}}$. I hope it is correct.\end{tabular}                                                                                                                                                                                                                                                 \\ \hline
Evaluate $\left\lceil\sqrt{27}\right\rceil - \left\lfloor\sqrt{26}\right\rfloor$.                                                                                                                                                                                                                                                                                                 & \begin{tabular}[c]{@{}l@{}}We have that $\left\lceil\sqrt{27}\right\rceil - \left\lfloor\sqrt{26}\right\rfloor = \left\lceil\sqrt{27}\right\rceil - \left\lfloor\sqrt{27}\right\rfloor = \boxed{1}$.\\ Final Answer: The final answer is $1$. I hope it is correct.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \hline
\begin{tabular}[c]{@{}l@{}}The sum of three numbers $a, b$ and $c$ is 88. \\ If we decrease $a$ by 5, we get $N$. If we increase $b$ by 5, we get $N$. If we multiply $c$ by 5, we get $N$. \\ What is the value of $N$?\end{tabular}                                                                                                                                             & \begin{tabular}[c]{@{}l@{}}Let $N=a+b+c$. Then, we have\\ \textbackslash{}begin\{align*\}\\ N-5a\&=b+c\textbackslash{}\textbackslash\\ N-5b\&=a+c\textbackslash{}\textbackslash\\ N-5c\&=a+b\textbackslash{}\textbackslash\\ \textbackslash{}end\{align*\}\\ Summing the above equations, we obtain\\ \\ $$b+c+a=N-5(a+b+c).$$\\ Adding $5(a+b+c)$ on both sides, we have\\ \\ $$N=5(a+b+c)+b+c+a.$$\\ Therefore, $N=\boxed{40}$.\\ Final Answer: The final answer is $40$. I hope it is correct.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \hline
\begin{tabular}[c]{@{}l@{}}Suppose $\frac ab = \frac35$,$\frac bc=\frac{15}6$, and $\frac cd = 6$. \\ What is the value of $\frac ad$? Express your answer in simplest form.\end{tabular}                                                                                                                                                                                         & \begin{tabular}[c]{@{}l@{}}The first equation tells us that $3b=5a$.  The second equation tells us that $3c=5d$.  \\ Therefore, $3b=5a$ and $3c=5d$, which implies that $b=5a$ and $c=5d$.  We can further simplify this to\\ \\ $$\textbackslash{}frac\{3b\}\{5a\}=\textbackslash{}frac\{3\}\{5\}c=\textbackslash{}frac\{3\}\{5\}\textbackslash{}cdot5d=\textbackslash{}frac\{15\}6\textbackslash{}cdot6=\textbackslash{}boxed\{9\}.$$\\ Final Answer: The final answer is $9$. I hope it is correct.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                            \\ \hline
\begin{tabular}[c]{@{}l@{}}Josh and Mike live 13 miles apart. \\ Yesterday Josh started to ride his bicycle toward Mike's house. \\ A little later Mike started to ride his bicycle toward Josh's house. \\ When they met, Josh had ridden for twice the length of time as Mike and at four-fifths of Mike's rate. \\ How many miles had  Mike ridden when they met?\end{tabular} & \begin{tabular}[c]{@{}l@{}}If Josh had ridden for twice the length of time as Mike, then Josh had ridden for a total of $2\cdot5=10$ miles. \\ If Mike had ridden for $x$ miles, then Mike had ridden for a total of $4x$ miles.  \\ Subtracting, we have $10=4x$. Therefore, $x=5$.\\ Final Answer: The final answer is $5$ miles. I hope it is correct.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
\begin{tabular}[c]{@{}l@{}}At her track meet, Alice ran at a speed of $9\ \text{m/s}$ for $12$ seconds. \\ How many meters did she run?\end{tabular}                                                                                                                                                                                                                              & \begin{tabular}[c]{@{}l@{}}We have that $v=9\text{ m/s}$, and we are given that the time is $12\text{ s}$.  We can therefore use the formula for distance:\\ $$\textbackslash{}begin\{align*\}\\ \textbackslash{}text\{Distance\} \&= \textbackslash{}text\{Speed\} \textbackslash{}times \textbackslash{}text\{Time\}\textbackslash{}\textbackslash\\ \textbackslash{}end\{align*\}$$\\ We then have that\\ $$\textbackslash{}begin\{align*\}\\ \textbackslash{}text\{Distance\} \&= 9 \textbackslash{}times \textbackslash{}text\{Time\}\textbackslash{}\textbackslash\\ \&=9\textbackslash{}times 12\textbackslash{}\textbackslash\\ \&=108\textbackslash{}text\{ m\}\\ \textbackslash{}end\{align*\}$$\\ Final Answer: The final answer is $108\text{ m}$. I hope it is correct.\end{tabular}                                                                                                                                                                                                                                                                              \\ \hline
\begin{tabular}[c]{@{}l@{}}The graph of the equation $y=ax^2+bx-6$ is completely below the $x$-axis. \\ If $a^2=49$, what is the largest possible integral value of $b$?\end{tabular}                                                                                                                                                                                             & \begin{tabular}[c]{@{}l@{}}For the equation to be completely below the $x$-axis, we need $y \le -6$, or $ax^2+bx-6 \le -6$. \\ Since $a^2=49$, $a>0$, so $a^2-6a+b \ge 0 \Rightarrow b \le 6a \Rightarrow b \le \boxed{12}$.\\ Final Answer: The final answer is $\boxed{12}$. I hope it is correct.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ \hline
\end{tabular}
}
\caption{Examples for CoTs from the Pythia model which we manually verified. All but one (the penultimate row) are wrong, while the final answer was deemed right by the verifier. }
\label{tab:cots}
\end{table*}
